Real-Time Rendering of Glinty Appearances using Distributed Binomial Laws on Anisotropic Grids

In this work, we render in real-time glittery materials caused by discrete flakes on the surface. To achieve this, one has to count the number of flakes reflecting the light towards the camera within every texel covered by a given pixel footprint. To do so, we derive a counting method for arbitrary footprints that, unlike previous work, outputs the correct statistics. We combine this counting method with an anisotropic parameterization of the texture space that reduces the number of texels falling under a pixel footprint. This allows our method to run with both stable performance and 1.5X to 5X faster than the state-of-the-art.

==> figures/fig_data_bernouilli_on_plane.tex <==
\begin{axis}[xmin=0.0,xmax=1.0,ymin=0.0,ymax=1.0,width=5.58cm,height=5.58cm,grid=both,]
    \addplot[mark=*,only marks,color=tab_orange,mark options={scale=0.6},forget plot,] coordinates {

(0.02395357158814311, 0.05522544147167818)
(0.19021235442627105, 0.06409459882409363)
(0.39442410756433705, 0.09917155953757743)
(0.6946398274578773, 0.11630309356071106)
(0.8949685457460632, 0.08195691132560164)
(0.12580334384053965, 0.18855998010489447)
(0.27545652034548396, 0.24888770479387906)
(0.4631675241890327, 0.15310529356639108)
(0.7133035009816809, 0.2275409574068988)
(0.7633803571247796, 0.1780682755627014)
(0.17939677092876033, 0.30055400444177355)
(0.49180935516085167, 0.32037457478638287)
(0.7756498128392431, 0.3112746997967716)
(0.062001823488654406, 0.47493154534886944)
(0.23321553338843704, 0.49257473942195257)
(0.2697653087754569, 0.42518291739645175)
(0.48892552646438714, 0.4324302959198675)
(0.5470906865174238, 0.49761831807643025)
(0.6586765456922291, 0.4405211989110509)
(0.010079910095053865, 0.5379079179556486)
(0.4414064948455909, 0.6173748020268119)
(0.9148478113264452, 0.5231962803765625)
(0.08976555066811703, 0.6382115917065052)
(0.20480483861935864, 0.6656589660680333)
(0.38106149029533964, 0.7086979228306501)
(0.5010121910708443, 0.7410466999689546)
(0.6284522170464781, 0.7451876483906661)
(0.3381659162896452, 0.869949431115559)
(0.44550832975638405, 0.8401884712486858)
(0.5917307215611238, 0.7628113596649686)
(0.7802288745990599, 0.7635445905447913)
(0.998998070927018, 0.8540059576293156)
(0.9192010151967533, 0.9165247888601346)
    };

    \addplot[mark=*,only marks,color=black,mark options={scale=0.6},forget plot,] coordinates {
(0.26992892323739615, 0.007379663842774553)
(0.5710154405625878, 0.032679097283797545)
(0.8429307535659418, 0.04640085186878304)
(0.1126191199634556, 0.14312307629969112)
(0.6031831806662448, 0.16887873067545445)
(0.9349514736558354, 0.15112527448069704)
(0.11744028342603466, 0.3423992651567013)
(0.2953394921977561, 0.26771344290703025)
(0.6241284597435753, 0.31194152413319975)
(0.7272907212989121, 0.3502369399485925)
(0.9671812497062736, 0.37034661533575164)
(0.8189131694897367, 0.4430033341052643)
(0.9226149415802538, 0.4808143324583799)
(0.24951296872325301, 0.5340084981424351)
(0.3131020968543212, 0.5286274407846259)
(0.5018622860793805, 0.5890640334669776)
(0.6976717463361146, 0.5580163256301829)
(0.8207918559532078, 0.5209914141277421)
(0.3325393310044313, 0.7406146693681763)
(0.7943003427876435, 0.7162995514825229)
(0.9954266065605245, 0.6412556800967745)
(0.05380214996465511, 0.7954640539606972)
(0.19747083819901623, 0.811453786337242)
(0.7357945353302956, 0.8184455585265815)
(0.007441143292269303, 0.8817512408987203)
(0.20303010784114003, 0.9205049802229859)
(0.33089286575609655, 0.9932820097729563)
(0.43776734547240753, 0.9951962721066663)
(0.5772933060609918, 0.8813921366450511)
(0.6804751953956416, 0.8801890747175231)
(0.8151420504433241, 0.9176065040571373)
    };

    \addplot[color=black,thick,fill=gray,fill opacity=0.125, opacity=0.25,forget plot,] coordinates {
        (0.00000, 0.00000)
        (0.75, 0.00000)
        (0.75, 0.75)
        (0.00000, 0.75)
    };

    \addplot[color=black,thick,fill=gray,fill opacity=0.5,forget plot,] coordinates {
        (0.00000, 0.00000)
        (0.5, 0.00000)
        (0.5, 0.5)
        (0.00000, 0.5)
    };

    \addplot[->,thick]
    coordinates {
        (1.00, 1.00)
        (0.75, 0.75)
    };
    \addplot[->,thick,opacity=0.25]
    coordinates {
        (1.00, 1.00)
        (0.50, 0.50)
    };

\end{axis}

==> figures/fig_data_blending_with_approx.tex <==
		\begin{scope}
		\begin{axis}[xmin=0.0,xmax=50.0,ymin=0.0,ymax=2000.0,width=5.58cm,height=5.58cm,grid=both,]
\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.125,opacity=0.25,forget plot,] coordinates {
				(0.00000, 0.00000)
				(1.00000, 0.00000)
				(2.00000, 0.00000)
				(3.00000, 0.00000)
				(4.00000, 0.00000)
				(5.00000, 0.00000)
				(6.00000, 0.00000)
				(7.00000, 0.00000)
				(8.00000, 0.00000)
				(9.00000, 0.00000)
				(10.00000, 0.00000)
				(11.00000, 0.00000)
				(12.00000, 0.00000)
				(13.00000, 0.00000)
				(14.00000, 0.00000)
				(15.00000, 0.00000)
				(16.00000, 1.00000)
				(17.00000, 0.00000)
				(18.00000, 2.00000)
				(19.00000, 1.00000)
				(20.00000, 14.00000)
				(21.00000, 24.00000)
				(22.00000, 36.00000)
				(23.00000, 75.00000)
				(24.00000, 140.00000)
				(25.00000, 206.00000)
				(26.00000, 313.00000)
				(27.00000, 437.00000)
				(28.00000, 591.00000)
				(29.00000, 789.00000)
				(30.00000, 893.00000)
				(31.00000, 924.00000)
				(32.00000, 1010.00000)
				(33.00000, 942.00000)
				(34.00000, 875.00000)
				(35.00000, 761.00000)
				(36.00000, 649.00000)
				(37.00000, 467.00000)
				(38.00000, 319.00000)
				(39.00000, 216.00000)
				(40.00000, 134.00000)
				(41.00000, 88.00000)
				(42.00000, 54.00000)
				(43.00000, 21.00000)
				(44.00000, 12.00000)
				(45.00000, 5.00000)
				(46.00000, 1.00000)
			};

			\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.125,opacity=0.25,forget plot,] coordinates {
				(0.00000, 0.00000)
				(1.00000, 2.00000)
				(2.00000, 20.00000)
				(3.00000, 86.00000)
				(4.00000, 269.00000)
				(5.00000, 640.00000)
				(6.00000, 1164.00000)
				(7.00000, 1728.00000)
				(8.00000, 2010.00000)
				(9.00000, 1773.00000)
				(10.00000, 1265.00000)
				(11.00000, 654.00000)
				(12.00000, 295.00000)
				(13.00000, 77.00000)
				(14.00000, 11.00000)
				(15.00000, 6.00000)
				(16.00000, 0.00000)
				(17.00000, 0.00000)
				(18.00000, 0.00000)
				(19.00000, 0.00000)
				(20.00000, 0.00000)
				(21.00000, 0.00000)
				(22.00000, 0.00000)
				(23.00000, 0.00000)
				(24.00000, 0.00000)
				(25.00000, 0.00000)
				(26.00000, 0.00000)
				(27.00000, 0.00000)
				(28.00000, 0.00000)
				(29.00000, 0.00000)
				(30.00000, 0.00000)
				(31.00000, 0.00000)
				(32.00000, 0.00000)
				(33.00000, 0.00000)
				(34.00000, 0.00000)
				(35.00000, 0.00000)
				(36.00000, 0.00000)
				(37.00000, 0.00000)
				(38.00000, 0.00000)
				(39.00000, 0.00000)
				(40.00000, 0.00000)
				(41.00000, 0.00000)
				(42.00000, 0.00000)
				(43.00000, 0.00000)
				(44.00000, 0.00000)
				(45.00000, 0.00000)
				(46.00000, 0.00000)
			};

			\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.5,forget plot,] coordinates {
				(0.00000, 0.00000)
				(1.00000, 0.00000)
				(2.00000, 0.00000)
				(3.00000, 0.00000)
				(4.00000, 0.00000)
				(5.00000, 0.00000)
				(6.00000, 0.00000)
				(7.00000, 1.00000)
				(8.00000, 3.00000)
				(9.00000, 18.00000)
				(10.00000, 44.00000)
				(11.00000, 99.00000)
				(12.00000, 196.00000)
				(13.00000, 386.00000)
				(14.00000, 585.00000)
				(15.00000, 833.00000)
				(16.00000, 1081.00000)
				(17.00000, 1269.00000)
				(18.00000, 1297.00000)
				(19.00000, 1242.00000)
				(20.00000, 1018.00000)
				(21.00000, 798.00000)
				(22.00000, 534.00000)
				(23.00000, 303.00000)
				(24.00000, 163.00000)
				(25.00000, 100.00000)
				(26.00000, 15.00000)
				(27.00000, 9.00000)
				(28.00000, 5.00000)
				(29.00000, 1.00000)
				(30.00000, 0.00000)
				(31.00000, 0.00000)
				(32.00000, 0.00000)
				(33.00000, 0.00000)
				(34.00000, 0.00000)
				(35.00000, 0.00000)
				(36.00000, 0.00000)
				(37.00000, 0.00000)
				(38.00000, 0.00000)
				(39.00000, 0.00000)
				(40.00000, 0.00000)
				(41.00000, 0.00000)
				(42.00000, 0.00000)
				(43.00000, 0.00000)
				(44.00000, 0.00000)
				(45.00000, 0.00000)
				(46.00000, 0.00000)
			};

			\addplot[thick,ybar interval,color=tab_blue,fill=tab_blue,fill opacity=0.5,forget plot,] coordinates {
				(0.00000, 0.00000)
				(1.00000, 0.00000)
				(2.00000, 0.00000)
				(3.00000, 0.00000)
				(4.00000, 0.00000)
				(5.00000, 0.00000)
				(6.00000, 0.00000)
				(7.00000, 1.00000)
				(8.00000, 1.00000)
				(9.00000, 8.00000)
				(10.00000, 39.00000)
				(11.00000, 50.00000)
				(12.00000, 136.00000)
				(13.00000, 268.00000)
				(14.00000, 493.00000)
				(15.00000, 747.00000)
				(16.00000, 1003.00000)
				(17.00000, 1176.00000)
				(18.00000, 1374.00000)
				(19.00000, 1288.00000)
				(20.00000, 1140.00000)
				(21.00000, 880.00000)
				(22.00000, 632.00000)
				(23.00000, 342.00000)
				(24.00000, 258.00000)
				(25.00000, 89.00000)
				(26.00000, 46.00000)
				(27.00000, 20.00000)
				(28.00000, 7.00000)
				(29.00000, 2.00000)
				(30.00000, 0.00000)
				(31.00000, 0.00000)
				(32.00000, 0.00000)
				(33.00000, 0.00000)
				(34.00000, 0.00000)
				(35.00000, 0.00000)
				(36.00000, 0.00000)
				(37.00000, 0.00000)
				(38.00000, 0.00000)
				(39.00000, 0.00000)
				(40.00000, 0.00000)
				(41.00000, 0.00000)
				(42.00000, 0.00000)
				(43.00000, 0.00000)
				(44.00000, 0.00000)
				(45.00000, 0.00000)
				(46.00000, 0.00000)
			};
		\end{axis}
	\end{scope}

==> figures/fig_data_histogram_Zirr.tex <==
	\begin{scope}  
		\begin{axis}[xmin=0.0,xmax=50.0,ymin=0.0,ymax=2000.0,width=5.58cm,height=5.58cm,grid=both,]
		\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.125,opacity=0.25,forget plot,] coordinates {
			(0.00000, 0.00000)
			(1.00000, 0.00000)
			(2.00000, 0.00000)
			(3.00000, 0.00000)
			(4.00000, 0.00000)
			(5.00000, 0.00000)
			(6.00000, 0.00000)
			(7.00000, 0.00000)
			(8.00000, 0.00000)
			(9.00000, 0.00000)
			(10.00000, 0.00000)
			(11.00000, 0.00000)
			(12.00000, 0.00000)
			(13.00000, 0.00000)
			(14.00000, 0.00000)
			(15.00000, 0.00000)
			(16.00000, 0.00000)
			(17.00000, 0.00000)
			(18.00000, 2.00000)
			(19.00000, 5.00000)
			(20.00000, 9.00000)
			(21.00000, 18.00000)
			(22.00000, 46.00000)
			(23.00000, 70.00000)
			(24.00000, 143.00000)
			(25.00000, 204.00000)
			(26.00000, 330.00000)
			(27.00000, 482.00000)
			(28.00000, 611.00000)
			(29.00000, 741.00000)
			(30.00000, 910.00000)
			(31.00000, 988.00000)
			(32.00000, 976.00000)
			(33.00000, 901.00000)
			(34.00000, 906.00000)
			(35.00000, 778.00000)
			(36.00000, 600.00000)
			(37.00000, 469.00000)
			(38.00000, 308.00000)
			(39.00000, 210.00000)
			(40.00000, 124.00000)
			(41.00000, 85.00000)
			(42.00000, 44.00000)
			(43.00000, 26.00000)
			(44.00000, 8.00000)
			(45.00000, 3.00000)
			(46.00000, 2.00000)
		};

		\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.125,opacity=0.25,forget plot,] coordinates {
			(0.00000, 0.00000)
			(1.00000, 2.00000)
			(2.00000, 26.00000)
			(3.00000, 79.00000)
			(4.00000, 285.00000)
			(5.00000, 684.00000)
			(6.00000, 1203.00000)
			(7.00000, 1729.00000)
			(8.00000, 1931.00000)
			(9.00000, 1752.00000)
			(10.00000, 1232.00000)
			(11.00000, 665.00000)
			(12.00000, 300.00000)
			(13.00000, 91.00000)
			(14.00000, 16.00000)
			(15.00000, 5.00000)
			(16.00000, 0.00000)
			(17.00000, 0.00000)
			(18.00000, 0.00000)
			(19.00000, 0.00000)
			(20.00000, 0.00000)
			(21.00000, 0.00000)
			(22.00000, 0.00000)
			(23.00000, 0.00000)
			(24.00000, 0.00000)
			(25.00000, 0.00000)
			(26.00000, 0.00000)
			(27.00000, 0.00000)
			(28.00000, 0.00000)
			(29.00000, 0.00000)
			(30.00000, 0.00000)
			(31.00000, 0.00000)
			(32.00000, 0.00000)
			(33.00000, 0.00000)
			(34.00000, 0.00000)
			(35.00000, 0.00000)
			(36.00000, 0.00000)
			(37.00000, 0.00000)
			(38.00000, 0.00000)
			(39.00000, 0.00000)
			(40.00000, 0.00000)
			(41.00000, 0.00000)
			(42.00000, 0.00000)
			(43.00000, 0.00000)
			(44.00000, 0.00000)
			(45.00000, 0.00000)
			(46.00000, 0.00000)
		};

		\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.5,forget plot,] coordinates {
			(0.00000, 0.00000)
			(1.00000, 0.00000)
			(2.00000, 0.00000)
			(3.00000, 0.00000)
			(4.00000, 0.00000)
			(5.00000, 0.00000)
			(6.00000, 0.00000)
			(7.00000, 3.00000)
			(8.00000, 7.00000)
			(9.00000, 18.00000)
			(10.00000, 48.00000)
			(11.00000, 103.00000)
			(12.00000, 204.00000)
			(13.00000, 357.00000)
			(14.00000, 589.00000)
			(15.00000, 890.00000)
			(16.00000, 1091.00000)
			(17.00000, 1182.00000)
			(18.00000, 1378.00000)
			(19.00000, 1195.00000)
			(20.00000, 1003.00000)
			(21.00000, 816.00000)
			(22.00000, 508.00000)
			(23.00000, 306.00000)
			(24.00000, 178.00000)
			(25.00000, 81.00000)
			(26.00000, 31.00000)
			(27.00000, 7.00000)
			(28.00000, 5.00000)
			(29.00000, 0.00000)
			(30.00000, 0.00000)
			(31.00000, 0.00000)
			(32.00000, 0.00000)
			(33.00000, 0.00000)
			(34.00000, 0.00000)
			(35.00000, 0.00000)
			(36.00000, 0.00000)
			(37.00000, 0.00000)
			(38.00000, 0.00000)
			(39.00000, 0.00000)
			(40.00000, 0.00000)
			(41.00000, 0.00000)
			(42.00000, 0.00000)
			(43.00000, 0.00000)
			(44.00000, 0.00000)
			(45.00000, 0.00000)
			(46.00000, 0.00000)
		};

		\addplot[thick,ybar interval,color=tab_green,fill=tab_green,fill opacity=0.5,forget plot,] coordinates {
			(0.00000, 0.00000)
			(1.00000, 0.00000)
			(2.00000, 0.00000)
			(3.00000, 0.00000)
			(4.00000, 0.00000)
			(5.00000, 0.00000)
			(6.00000, 0.00000)
			(7.00000, 0.00000)
			(8.00000, 0.00000)
			(9.00000, 0.00000)
			(10.00000, 0.00000)
			(11.00000, 1.00000)
			(12.00000, 3.00000)
			(13.00000, 18.00000)
			(14.00000, 80.00000)
			(15.00000, 196.00000)
			(16.00000, 445.00000)
			(17.00000, 856.00000)
			(18.00000, 1292.00000)
			(19.00000, 1666.00000)
			(20.00000, 1786.00000)
			(21.00000, 1475.00000)
			(22.00000, 1072.00000)
			(23.00000, 657.00000)
			(24.00000, 300.00000)
			(25.00000, 103.00000)
			(26.00000, 41.00000)
			(27.00000, 6.00000)
			(28.00000, 3.00000)
			(29.00000, 0.00000)
			(30.00000, 0.00000)
			(31.00000, 0.00000)
			(32.00000, 0.00000)
			(33.00000, 0.00000)
			(34.00000, 0.00000)
			(35.00000, 0.00000)
			(36.00000, 0.00000)
			(37.00000, 0.00000)
			(38.00000, 0.00000)
			(39.00000, 0.00000)
			(40.00000, 0.00000)
			(41.00000, 0.00000)
			(42.00000, 0.00000)
			(43.00000, 0.00000)
			(44.00000, 0.00000)
			(45.00000, 0.00000)
			(46.00000, 0.00000)
		};

	\end{axis}
\end{scope}

==> figures/fig_data_histogram_true.tex <==
	\begin{scope}
		\begin{axis}[xmin=0.0,xmax=50.0,ymin=0.0,ymax=2000.0,width=5.58cm,height=5.58cm,grid=both,]
		\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.125,opacity=0.25,forget plot,] coordinates {
			(0.00000, 0.00000)
			(1.00000, 0.00000)
			(2.00000, 0.00000)
			(3.00000, 0.00000)
			(4.00000, 0.00000)
			(5.00000, 0.00000)
			(6.00000, 0.00000)
			(7.00000, 0.00000)
			(8.00000, 0.00000)
			(9.00000, 0.00000)
			(10.00000, 0.00000)
			(11.00000, 0.00000)
			(12.00000, 0.00000)
			(13.00000, 0.00000)
			(14.00000, 0.00000)
			(15.00000, 0.00000)
			(16.00000, 1.00000)
			(17.00000, 0.00000)
			(18.00000, 4.00000)
			(19.00000, 4.00000)
			(20.00000, 10.00000)
			(21.00000, 33.00000)
			(22.00000, 43.00000)
			(23.00000, 101.00000)
			(24.00000, 136.00000)
			(25.00000, 185.00000)
			(26.00000, 320.00000)
			(27.00000, 431.00000)
			(28.00000, 623.00000)
			(29.00000, 715.00000)
			(30.00000, 897.00000)
			(31.00000, 971.00000)
			(32.00000, 1004.00000)
			(33.00000, 966.00000)
			(34.00000, 950.00000)
			(35.00000, 718.00000)
			(36.00000, 630.00000)
			(37.00000, 444.00000)
			(38.00000, 294.00000)
			(39.00000, 213.00000)
			(40.00000, 133.00000)
			(41.00000, 86.00000)
			(42.00000, 45.00000)
			(43.00000, 20.00000)
			(44.00000, 15.00000)
			(45.00000, 6.00000)
			(46.00000, 2.00000)
		};

		\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.125,opacity=0.25,forget plot,] coordinates {
			(0.00000, 2.00000)
			(1.00000, 20.00000)
			(2.00000, 70.00000)
			(3.00000, 226.00000)
			(4.00000, 525.00000)
			(5.00000, 890.00000)
			(6.00000, 1239.00000)
			(7.00000, 1459.00000)
			(8.00000, 1512.00000)
			(9.00000, 1335.00000)
			(10.00000, 999.00000)
			(11.00000, 722.00000)
			(12.00000, 492.00000)
			(13.00000, 248.00000)
			(14.00000, 137.00000)
			(15.00000, 69.00000)
			(16.00000, 39.00000)
			(17.00000, 5.00000)
			(18.00000, 7.00000)
			(19.00000, 3.00000)
			(20.00000, 0.00000)
			(21.00000, 1.00000)
			(22.00000, 0.00000)
			(23.00000, 0.00000)
			(24.00000, 0.00000)
			(25.00000, 0.00000)
			(26.00000, 0.00000)
			(27.00000, 0.00000)
			(28.00000, 0.00000)
			(29.00000, 0.00000)
			(30.00000, 0.00000)
			(31.00000, 0.00000)
			(32.00000, 0.00000)
			(33.00000, 0.00000)
			(34.00000, 0.00000)
			(35.00000, 0.00000)
			(36.00000, 0.00000)
			(37.00000, 0.00000)
			(38.00000, 0.00000)
			(39.00000, 0.00000)
			(40.00000, 0.00000)
			(41.00000, 0.00000)
			(42.00000, 0.00000)
			(43.00000, 0.00000)
			(44.00000, 0.00000)
			(45.00000, 0.00000)
			(46.00000, 0.00000)
		};

		\addplot[thick,ybar interval,color=tab_orange,fill=tab_orange,fill opacity=0.5,forget plot,] coordinates {
			(0.00000, 0.00000)
			(1.00000, 0.00000)
			(2.00000, 0.00000)
			(3.00000, 0.00000)
			(4.00000, 0.00000)
			(5.00000, 2.00000)
			(6.00000, 0.00000)
			(7.00000, 6.00000)
			(8.00000, 21.00000)
			(9.00000, 48.00000)
			(10.00000, 119.00000)
			(11.00000, 165.00000)
			(12.00000, 314.00000)
			(13.00000, 458.00000)
			(14.00000, 696.00000)
			(15.00000, 861.00000)
			(16.00000, 989.00000)
			(17.00000, 1059.00000)
			(18.00000, 1093.00000)
			(19.00000, 1023.00000)
			(20.00000, 930.00000)
			(21.00000, 701.00000)
			(22.00000, 545.00000)
			(23.00000, 376.00000)
			(24.00000, 279.00000)
			(25.00000, 144.00000)
			(26.00000, 74.00000)
			(27.00000, 45.00000)
			(28.00000, 29.00000)
			(29.00000, 11.00000)
			(30.00000, 9.00000)
			(31.00000, 1.00000)
			(32.00000, 1.00000)
			(33.00000, 0.00000)
			(34.00000, 1.00000)
			(35.00000, 0.00000)
			(36.00000, 0.00000)
			(37.00000, 0.00000)
			(38.00000, 0.00000)
			(39.00000, 0.00000)
			(40.00000, 0.00000)
			(41.00000, 0.00000)
			(42.00000, 0.00000)
			(43.00000, 0.00000)
			(44.00000, 0.00000)
			(45.00000, 0.00000)
			(46.00000, 0.00000)
		};

		\addplot[thick,ybar interval,color=tab_blue,fill=tab_blue,fill opacity=0.5,forget plot,] coordinates {
			(0.00000, 0.00000)
			(1.00000, 0.00000)
			(2.00000, 0.00000)
			(3.00000, 0.00000)
			(4.00000, 0.00000)
			(5.00000, 0.00000)
			(6.00000, 1.00000)
			(7.00000, 8.00000)
			(8.00000, 30.00000)
			(9.00000, 37.00000)
			(10.00000, 80.00000)
			(11.00000, 159.00000)
			(12.00000, 277.00000)
			(13.00000, 430.00000)
			(14.00000, 621.00000)
			(15.00000, 787.00000)
			(16.00000, 910.00000)
			(17.00000, 1007.00000)
			(18.00000, 1018.00000)
			(19.00000, 980.00000)
			(20.00000, 893.00000)
			(21.00000, 745.00000)
			(22.00000, 661.00000)
			(23.00000, 461.00000)
			(24.00000, 321.00000)
			(25.00000, 221.00000)
			(26.00000, 141.00000)
			(27.00000, 96.00000)
			(28.00000, 60.00000)
			(29.00000, 29.00000)
			(30.00000, 17.00000)
			(31.00000, 6.00000)
			(32.00000, 2.00000)
			(33.00000, 1.00000)
			(34.00000, 1.00000)
			(35.00000, 0.00000)
			(36.00000, 0.00000)
			(37.00000, 0.00000)
			(38.00000, 0.00000)
			(39.00000, 0.00000)
			(40.00000, 0.00000)
			(41.00000, 0.00000)
			(42.00000, 0.00000)
			(43.00000, 0.00000)
			(44.00000, 0.00000)
			(45.00000, 0.00000)
			(46.00000, 0.00000)
		};

	\end{axis}
\end{scope}


==> figures/lst_algorithm.tex <==
\definecolor{lstbackground}{rgb}{0.1, 0.1, 0.1}
\definecolor{lstbasic}{rgb}{1, 1, 1}
\definecolor{lstframe}{gray}{0.80}
\definecolor{lstcomment}{rgb}{0.41, 0.59, 0.33}
\definecolor{lstkeyword}{rgb}{0.85, 0.85, 0.61}
\definecolor{lstnumber}{rgb}{0.5, 0.0, 0.0}
\definecolor{lstattrib}{rgb}{0,0.34,0}
\definecolor{lstvariable}{rgb}{0.6,0.85,0.98}
\lstset{
    language=C,
    basicstyle = \scriptsize\ttfamily\raggedright\color{lstbasic},
    stringstyle=\color{lstattrib},
    mathescape = true,
    frame = lrtb,
    % backgroundcolor = \color{lstbackground},
    % rulecolor = \color{lstframe},
    tabsize = 3,
    columns = fullflexible,
    keepspaces,
    belowskip = \smallskipamount,
    framerule = 0.0pt,
    breaklines = true,
    showstringspaces = false,
    captionpos = t,
    texcl=false,
    keywords={with,sum,mean,no_grad,rand,return,def,backward,step,for},
    keywordstyle=\color{lstkeyword}\bfseries, 
    commentstyle=\color{lstcomment}\itshape\bfseries,
    identifierstyle=\color{lstvariable}\bfseries,
    numberstyle = \color{lstnumber}\bfseries,
    caption={
        High-level pseudocode overview of our full glinty NDF evaluation algorithm.
    },
    label={lst:algorithm},
    captionpos=b
}
\begin{tcolorbox}[colback=black,
                  %breakable,
                  nobeforeafter, 
                  left=5pt,
                  right=-10pt,
                  top=0pt,
                  bottom=-1.2cm,
                  ]
\begin{lstlisting}
// Algorithm inputs
texture coordinates UV
halfvector slope S
target NDF function D()
microfacet density d
microfacet density variance dV
glitteriness ratio parameter R

// Glinty NDF parameters
p = D(S) / D(0) * R
GS = discretize slope space into grid with stride R

// Evaluate distributed binomial law on anisotropic grids
P = compute pixel ellipse footprint from dFdx(UV), dFdy(UV)
G[...] = discrete anisotropic parameterizations around P
wG[...] = aniso. param. blending weight for G[...]
N[...] = d * cell_area(G[...])
for i in size(G):
    // Transform UV based on G[i] parameterization
    UVg = scale(stretch(rotate(UV)))  
    // Find surface grid cell in G[i]
    T[...] = texels surrounding UVg in G[i]
    wT[...] = texel blending weight for T[...]  
    for j in size(T):
        // Randomize microfacet density for this texel
        seedDV = rand(G[i], T[j])
        M = sample_gaussian(seedDV, N[i], dV)     
        // Find angular cell in slope space grid GS
        V[...] = texels surrounding S in GS
        wV[...] = texel blending weight for V[...]      
        for k in size(V):
            // Sample binomial for this angular texel
            seedB = rand(G[i], T[j], V[k])
            X[k] = binomial(seedB, M * wG[i], p) / M
        // Interpolate all angular texel results
        Y[j] = sum(X[...] * wV[...])
    // Interpolate all surface texel results
    Z[i] = sum(Y[...] * wT[...])
// Sum up all anisotropic grid results
binomial = sum(Z[...])

// Evaluate glinty NDF
NDF = binomial * D(0) / R
\end{lstlisting}
\end{tcolorbox}

==> figures/lst_algorithm2.tex <==
\definecolor{lstbackground}{rgb}{0.1, 0.1, 0.1}
\definecolor{lstbasic}{rgb}{1, 1, 1}
\definecolor{lstframe}{gray}{0.80}
\definecolor{lstcomment}{rgb}{0.41, 0.59, 0.33}
\definecolor{lstkeyword}{rgb}{0.85, 0.85, 0.61}
\definecolor{lstnumber}{rgb}{0.5, 0.0, 0.0}
\definecolor{lstattrib}{rgb}{0,0.34,0}
\definecolor{lstvariable}{rgb}{0.6,0.85,0.98}
\lstset{
    language=C,
    basicstyle = \scriptsize\ttfamily\raggedright\color{lstbasic},
    stringstyle=\color{lstattrib},
    mathescape = true,
    frame = lrtb,
    % backgroundcolor = \color{lstbackground},
    % rulecolor = \color{lstframe},
    tabsize = 3,
    columns = fullflexible,
    keepspaces,
    belowskip = \smallskipamount,
    framerule = 0.0pt,
    breaklines = true,
    showstringspaces = false,
    captionpos = t,
    texcl=false,
    keywords={with,sum,mean,no_grad,rand,return,def,backward,step,for},
    keywordstyle=\color{lstkeyword}\bfseries, 
    commentstyle=\color{lstcomment}\itshape\bfseries,
    identifierstyle=\color{lstvariable}\bfseries,
    numberstyle = \color{lstnumber}\bfseries,
    caption={
        High-level pseudocode overview of our full glinty NDF evaluation algorithm.
    },
    label={lst:algorithm},
    captionpos=b
}
\begin{tcolorbox}[colback=black,
                  %breakable,
                  nobeforeafter, 
                  left=5pt,
                  right=-10pt,
                  top=0pt,
                  bottom=-1.2cm,
                  ]
\begin{lstlisting}
// Algorithm inputs
texture coordinates UV
pixel footprint P
halfvector slope S
target NDF function D()
glitteriness ratio parameter R

// Binomial p parameter
p = D(S) / D(0) * R

// Evaluate distributed binomial law on anisotropic grids
find anisotropic surface grids G[0...3] around P
compute associated microfacet counts N[0...3]
compute associated blending weights w[0...3]
for i in [0...3]:
    find surface simplex cell C around UV in G[i]
    find vertices V[0...2] of simplex cell C
    for j in [0...2]:
        discretize slope space into grid Gs using stride R
        find angular bilinear cell D around S in Gs
        find vertices U[0...3] of bilinear cell D    
        // This loop is parallelized into four-component SIMD
        for k in [0...3]:
            seed = rand(G[i], V[j], U[k])
            X[k] = binomial(seed, N[i] * w[i], p) / N[i]
        Y[j] = bilinear interpolation of X[0...3]
    Z[i] = barycentric simplex interpolation of Y[0...2]
binomial = Z[0] + Z[1] + Z[2] + Z[3]

// Evaluate glinty NDF
ndf = binomial * D(0) / R  
\end{lstlisting}
\end{tcolorbox}
